{\mu}-cuDNN: Accelerating Deep Learning Frameworks with Micro-Batching

NVIDIA cuDNN is a low-level library that provides GPU kernels frequently used in deep learning. Specifically, cuDNN implements several equivalent convolution algorithms, whose performance and memory footprint may vary considerably, depending on the layer dimensions. When an algorithm is automatically selected by cuDNN, the decision is performed on a per-layer basis, and thus it often resorts to slower algorithms that fit the workspace size constraints. We present {\mu}-cuDNN, a transparent wrapper library for cuDNN, which divides layers' mini-batch computation into several micro-batches. Based on Dynamic Programming and Integer Linear Programming, {\mu}-cuDNN enables faster algorithms by decreasing the workspace requirements. At the same time, {\mu}-cuDNN keeps the computational semantics unchanged, so that it decouples statistical efficiency from the hardware efficiency safely. We demonstrate the effectiveness of {\mu}-cuDNN over two frameworks, Caffe and TensorFlow, achieving speedups of 1.63x for AlexNet and 1.21x for ResNet-18 on P100-SXM2 GPU. These results indicate that using micro-batches can seamlessly increase the performance of deep learning, while maintaining the same memory footprint.

==> performance.tex <==
\makeatletter

%%% script/caffe_time_layer

\@namedef{caffe-time-layer-alexnet-p100-64mb-conv2-forward-gemm-ws}{4.3 KiB}
\@namedef{caffe-time-layer-alexnet-p100-64mb-conv2-forward-fft-ws-u32}{48.9 MiB}
\@namedef{caffe-time-layer-alexnet-p100-64mb-conv2-forward-fft-ws}{213 MiB}
\@namedef{caffe-time-layer-alexnet-p100-64mb-conv2-forward-speedup}{2.33}
% [1] 2.331425
% $undivided
%      lib algo batch memory     time
% 8 ucudnn    1   256   4380 6.280896

% $powerOfTwo
%       lib algo batch   memory     time
% 8  ucudnn    5    32 51273728 0.375424
% 9  ucudnn    5    32 51273728 0.375424
% 10 ucudnn    5    32 51273728 0.375424
% 11 ucudnn    5    32 51273728 0.375424
% 12 ucudnn    5    32 51273728 0.375424
% 13 ucudnn    5    32 51273728 0.375424
% 14 ucudnn    5    32 51273728 0.375424
% 15 ucudnn    5    32 51273728 0.375424

% $all
%       lib algo batch   memory     time
% 14 ucudnn    5    32 51273728 0.356672
% 15 ucudnn    5    32 51273728 0.356672
% 16 ucudnn    7    48 55550976 0.495168
% 17 ucudnn    7    48 55550976 0.495168
% 18 ucudnn    7    48 55550976 0.495168
% 19 ucudnn    7    48 55550976 0.495168


%%% script/caffe_time %%%

\@namedef{caffe-time-alexnet-k80-64mb-speedup}{1.81}
\@namedef{caffe-time-alexnet-k80-64mb-speedup-conv}{2.10}

\@namedef{caffe-time-alexnet-p100-64mb-speedup}{1.40}
\@namedef{caffe-time-alexnet-p100-64mb-speedup-conv}{1.63}
\@namedef{caffe-time-alexnet-p100-64mb-slowdown-conv-to-512mb-undivided}{1.17} % 79.56774 / 68.16955

\@namedef{caffe-time-alexnet-v100-64mb-speedup}{1.47}
\@namedef{caffe-time-alexnet-v100-64mb-speedup-conv}{1.63}

\@namedef{caffe-time-resnet18-p100-64mb-speedup}{1.11}
\@namedef{caffe-time-resnet18-p100-64mb-speedup-conv}{1.21}
\@namedef{caffe-time-resnet18-p100-64mb-slowdown-to-512mb-undivided-conv}{1.07} % 134.8159 / 125.8071

\@namedef{caffe-time-resnet18-v100-64mb-speedup}{1.22}
\@namedef{caffe-time-resnet18-v100-64mb-speedup-conv}{1.30}

\@namedef{caffe-time-alexnet-p100-64mb-ws-all}{0.70 GiB}
\@namedef{caffe-time-alexnet-p100-512mb-ws-undivided}{2.87 GiB}
% cat script/caffe_time/log/p100_smx2_tsubame3/log_512mb_alexnet_ucudnn_undivided
%  | grep util | sed "s/.*(\([^\[]*\).*/\1/g"

\@namedef{caffe-time-alexnet-p100-64mb-speedup-512mb-undivided}{1.04} % 122.8011 / 118.6428
\@namedef{caffe-time-alexnet-p100-64mb-speedup-512mb-undivided-percent}{4\%}


%%% script/caffe_time_wdiv %%%

\@namedef{caffe-time-wdiv-alexnet-p100-120mb-speedup}{1.24}
\@namedef{caffe-time-wdiv-alexnet-p100-120mb-speedup-conv}{1.38}
\@namedef{caffe-time-wdiv-alexnet-p100-120mb-speedup-960mb-baseline}{1.24} % 172.09746298 / 138.3612447
% Baseline (undivided (WR, 8 MiB)): 172.12822502 (129.84536)
% WD (all (WD, 120 MiB)): 138.3612447 (93.80884)
% Speedup: 1.24 (1.38)
% ---
% Baseline (undivided (WR, 64 MiB)): 172.09746298 (129.87995)
% WD (all (WD, 960 MiB)): 116.87987888 (73.66079)
% Speedup: 1.47 (1.76)
% ---
% Baseline (undivided (WR, 512 MiB)): 118.64278016 (68.16955)
% WD (all (WD, 7680 MiB)): 113.18721288 (65.22611)
% Speedup: 1.05 (1.05)

\@namedef{caffe-time-wdiv-resnet50-p100-2544mb-speedup}{1.05}
\@namedef{caffe-time-wdiv-resnet50-p100-2544mb-speedup-conv}{1.14}
% Baseline (undivided (WR, 8 MiB)): 241.09613254 (105.298418)
% WD (all (WD, 1272 MiB)): 229.40224178 (93.580094)
% Speedup: 1.05 (1.13)
% ---
% Baseline (undivided (WR, 16 MiB)): 240.5640735 (104.879498)
% WD (all (WD, 2544 MiB)): 228.0574079 (92.305338)
% Speedup: 1.05 (1.14)
% ---
% Baseline (undivided (WR, 32 MiB)): 240.82215756 (104.975924)
% WD (all (WD, 5088 MiB)): 228.6290244 (92.842155)
% Speedup: 1.05 (1.13)


%%% script/caffe_time_alexnet_ws %%%

\@namedef{caffe-time-alexnet-ws-120mb-prop-conv2-conv3}{93.7\%}
\@namedef{caffe-time-alexnet-ws-120mb-ws-max-conv4-conv5}{3 MiB}

\@namedef{caffe-time-alexnet-ws-120mb-conv5-forward-best-ws}{109 MiB}
\@namedef{caffe-time-alexnet-ws-120mb-conv5-forward-best-speedup}{1.29}
%% from script/caffe_time_wdiv/log/p100_smx2_tsubame3/log_120mb_alexnet_ucudnn_all
% --- Convolutional layer optimization using DP (Forward, [256,192,13,13] -> [256,128,13,13] (3x3, pad 1x1)) ---
% Batch size policy: all
% Maximum workspace size: 125829120
% Time to benchmark all existing kernels: 1707802[us]
% Time to optimize combination of kernels using DP: 340853[us]
% Number of optimized configuration sets: 10
% Best cuDNN kernel: {algo: 6, micro-batch: 256, workspace: 1572864, time: 1.735968}
% ---
% Desirable u-cuDNN kernel(s): {algo: 4, micro-batch: 128, workspace: 114130944, time: 0.670784}
%                         {algo: 4, micro-batch: 128, workspace: 114130944, time: 0.670784}
% Expected speedup: 1.29398 (1.73597[ms] -> 1.34157[ms])
% Workspace size ratio: 72.5625 (1572864[bytes] -> 114130944[bytes])
% Workspace utilization: 0.907031 (114130944[bytes] / 125829120[bytes])


%%% script/caffe_time_benchmark_time %%%
\@namedef{caffe-time-alexnet-p100-64mb-benchmark-all}{34.16 s}
\@namedef{caffe-time-alexnet-p100-64mb-benchmark-poweroftwo}{3.82 s}


%%% script/tensorflow_time %%%
\@namedef{tf-time-alexnet-p100-64mb-speedup}{1.24}
\@namedef{tf-time-resnet50-p100-64mb-speedup}{1.06}


%%% script/forward_memory_consumption
\@namedef{forward-memory-consumption-ratio-max-alexnet}{3.43}
\@namedef{forward-memory-consumption-ratio-max-resnet18}{2.73}

\newcommand{\perf}[1]{\@nameuse{#1}}
% \newcommand{\perf}[1]{\textcolor{cyan}{\fbox{\@nameuse{#1}}}}
\makeatother

